Generative AI Misuse: A Taxonomy of Tactics and Insights from Real-World Data

Generative, multimodal artificial intelligence (GenAI) offers transformative potential across industries, but its misuse poses significant risks. Prior research has shed light on the potential of advanced AI systems to be exploited for malicious purposes. However, we still lack a concrete understanding of how GenAI models are specifically exploited or abused in practice, including the tactics employed to inflict harm. In this paper, we present a taxonomy of GenAI misuse tactics, informed by existing academic literature and a qualitative analysis of approximately 200 observed incidents of misuse reported between January 2023 and March 2024. Through this analysis, we illuminate key and novel patterns in misuse during this time period, including potential motivations, strategies, and how attackers leverage and abuse system capabilities across modalities (e.g. image, text, audio, video) in the wild.

==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> references.tex <==


@article{dufour2024ammeba,
  title={AMMeBa: A Large-Scale Survey and Dataset of Media-Based Misinformation In-The-Wild},
  author={Dufour, Nicholas and Pathak, Arkanath and Samangouei, Pouya and Hariri, Nikki and Deshetti, Shashi and Dudfield, Andrew and Guess, Christopher and Escayola, Pablo Hern{\'a}ndez and Tran, Bobby and Babakar, Mevan and others},
  url           = "http://arxiv.org/abs/2405.11697",
  archivePrefix = "arXiv",
  eprint        = "2405.11697",
  primaryClass  = "cs.CL",
  arxivid       = "2405.11697",
  doi           = "10.48550/arXiv.2405.11697",
  year={2024}
}



@ARTICLE{Betker2023-ij,
  title    = "Improving image generation with better captions",
  author   = "Betker, James and Goh, Gabriel and Jing, Li and Brooks, Tim and
              Jianfeng, Wang and Li, Linjie and Ouyang, Long and Zhuang,
              Juntang and Lee, Joyce and Guo, Yufei and Manassra, Wesam and
              Dhariwal, Prafulla and Chu, Casey and Jiao, Yunxin and Ramesh,
              Aditya",
  abstract = "We show that prompt following abilities of text-to-image models
              can be substantially improved by training on highly descriptive
              generated image captions. Existing text-to-image models struggle
              to follow detailed image descriptions and often ignore words or
              confuse the meaning of prompts. We hypothesize that this issue
              stems from noisy and inaccurate image captions in the training
              dataset. We address this by training a bespoke image captioner
              and use it to recaption the training dataset. We then train
              several text-to-image models and find that training on these
              synthetic captions reliably improves prompt following ability.
              Finally, we use these findings to build DALL-E 3: a new
              text-to-image generation system, and benchmark its performance on
              an evaluation designed to measure prompt following, coherence,
              and aesthetics, finding that it compares favorably to
              competitors. We publish samples and code for these evaluations so
              that future research can continue optimizing this important
              aspect of text-to-image systems.",
  month    =  oct,
  year     =  2023,
  url      = "https://cdn.openai.com/papers/dall-e-3.pdf"
}

@ARTICLE{Carlini2024-zu,
  title         = "Stealing Part of a Production Language Model",
  author        = "Carlini, Nicholas and Paleka, Daniel and Dvijotham,
                   Krishnamurthy Dj and Steinke, Thomas and Hayase, Jonathan
                   and Feder Cooper, A and Lee, Katherine and Jagielski,
                   Matthew and Nasr, Milad and Conmy, Arthur and Wallace, Eric
                   and Rolnick, David and Tram{\`e}r, Florian",
  abstract      = "We introduce the first model-stealing attack that extracts
                   precise, nontrivial information from black-box production
                   language models like OpenAI's ChatGPT or Google's PaLM-2.
                   Specifically, our attack recovers the embedding projection
                   layer (up to symmetries) of a transformer model, given
                   typical API access. For under \$20 USD, our attack extracts
                   the entire projection matrix of OpenAI's Ada and Babbage
                   language models. We thereby confirm, for the first time,
                   that these black-box models have a hidden dimension of 1024
                   and 2048, respectively. We also recover the exact hidden
                   dimension size of the gpt-3.5-turbo model, and estimate it
                   would cost under \$2,000 in queries to recover the entire
                   projection matrix. We conclude with potential defenses and
                   mitigations, and discuss the implications of possible future
                   work that could extend our attack.",
  month         =  mar,
  year          =  2024,
  url           = "http://arxiv.org/abs/2403.06634",
  archivePrefix = "arXiv",
  eprint        = "2403.06634",
  primaryClass  = "cs.CR",
  arxivid       = "2403.06634",
  doi           = "10.48550/arXiv.2403.06634"
}

@ARTICLE{Sadasivan2023-mv,
  title         = "Can {AI-Generated} Text be Reliably Detected?",
  author        = "Sadasivan, Vinu Sankar and Kumar, Aounon and
                   Balasubramanian, Sriram and Wang, Wenxiao and Feizi, Soheil",
  abstract      = "The unregulated use of LLMs can potentially lead to
                   malicious consequences such as plagiarism, generating fake
                   news, spamming, etc. Therefore, reliable detection of
                   AI-generated text can be critical to ensure the responsible
                   use of LLMs. Recent works attempt to tackle this problem
                   either using certain model signatures present in the
                   generated text outputs or by applying watermarking
                   techniques that imprint specific patterns onto them. In this
                   paper, we show that these detectors are not reliable in
                   practical scenarios. In particular, we develop a recursive
                   paraphrasing attack to apply on AI text, which can break a
                   whole range of detectors, including the ones using the
                   watermarking schemes as well as neural network-based
                   detectors, zero-shot classifiers, and retrieval-based
                   detectors. Our experiments include passages around 300
                   tokens in length, showing the sensitivity of the detectors
                   even in the case of relatively long passages. We also
                   observe that our recursive paraphrasing only degrades text
                   quality slightly, measured via human studies, and metrics
                   such as perplexity scores and accuracy on text benchmarks.
                   Additionally, we show that even LLMs protected by
                   watermarking schemes can be vulnerable against spoofing
                   attacks aimed to mislead detectors to classify human-written
                   text as AI-generated, potentially causing reputational
                   damages to the developers. In particular, we show that an
                   adversary can infer hidden AI text signatures of the LLM
                   outputs without having white-box access to the detection
                   method. Finally, we provide a theoretical connection between
                   the AUROC of the best possible detector and the Total
                   Variation distance between human and AI text distributions
                   that can be used to study the fundamental hardness of the
                   reliable detection problem for advanced language models. Our
                   code is publicly available at
                   https://github.com/vinusankars/Reliability-of-AI-text-detectors.",
  month         =  mar,
  year          =  2023,
  url           = "http://arxiv.org/abs/2303.11156",
  archivePrefix = "arXiv",
  eprint        = "2303.11156",
  primaryClass  = "cs.CL",
  arxivid       = "2303.11156",
  doi           = "10.48550/arXiv.2303.11156"
}

@ARTICLE{DiResta2024-hs,
  title         = "How Spammers and Scammers Leverage {AI-Generated} Images on
                   Facebook for Audience Growth",
  author        = "DiResta, Renee and Goldstein, Josh A",
  abstract      = "Much of the research and discourse on risks from artificial
                   intelligence (AI) image generators, such as DALL-E and
                   Midjourney, has centered around whether they could be used
                   to inject false information into political discourse. We
                   show that spammers and scammers - seemingly motivated by
                   profit or clout, not ideology - are already using
                   AI-generated images to gain significant traction on
                   Facebook. At times, the Facebook Feed is recommending
                   unlabeled AI-generated images to users who neither follow
                   the Pages posting the images nor realize that the images are
                   AI-generated, highlighting the need for improved
                   transparency and provenance standards as AI models
                   proliferate.",
  month         =  mar,
  year          =  2024,
  url           = "http://arxiv.org/abs/2403.12838",
  archivePrefix = "arXiv",
  eprint        = "2403.12838",
  primaryClass  = "cs.CY",
  arxivid       = "2403.12838",
  doi           = "10.48550/arXiv.2403.12838"
}

@ARTICLE{Touvron2023-sv,
  title         = "Llama 2: Open Foundation and {Fine-Tuned} Chat Models",
  author        = "Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert,
                   Peter and Almahairi, Amjad and Babaei, Yasmine and
                   Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal
                   and Bhosale, Shruti and Bikel, Dan and Blecher, Lukas and
                   Ferrer, Cristian Canton and Chen, Moya and Cucurull, Guillem
                   and Esiobu, David and Fernandes, Jude and Fu, Jeremy and Fu,
                   Wenyin and Fuller, Brian and Gao, Cynthia and Goswami,
                   Vedanuj and Goyal, Naman and Hartshorn, Anthony and
                   Hosseini, Saghar and Hou, Rui and Inan, Hakan and Kardas,
                   Marcin and Kerkez, Viktor and Khabsa, Madian and Kloumann,
                   Isabel and Korenev, Artem and Koura, Punit Singh and
                   Lachaux, Marie-Anne and Lavril, Thibaut and Lee, Jenya and
                   Liskovich, Diana and Lu, Yinghai and Mao, Yuning and
                   Martinet, Xavier and Mihaylov, Todor and Mishra, Pushkar and
                   Molybog, Igor and Nie, Yixin and Poulton, Andrew and
                   Reizenstein, Jeremy and Rungta, Rashi and Saladi, Kalyan and
                   Schelten, Alan and Silva, Ruan and Smith, Eric Michael and
                   Subramanian, Ranjan and Tan, Xiaoqing Ellen and Tang, Binh
                   and Taylor, Ross and Williams, Adina and Kuan, Jian Xiang
                   and Xu, Puxin and Yan, Zheng and Zarov, Iliyan and Zhang,
                   Yuchen and Fan, Angela and Kambadur, Melanie and Narang,
                   Sharan and Rodriguez, Aurelien and Stojnic, Robert and
                   Edunov, Sergey and Scialom, Thomas",
  abstract      = "In this work, we develop and release Llama 2, a collection
                   of pretrained and fine-tuned large language models (LLMs)
                   ranging in scale from 7 billion to 70 billion parameters.
                   Our fine-tuned LLMs, called Llama 2-Chat, are optimized for
                   dialogue use cases. Our models outperform open-source chat
                   models on most benchmarks we tested, and based on our human
                   evaluations for helpfulness and safety, may be a suitable
                   substitute for closed-source models. We provide a detailed
                   description of our approach to fine-tuning and safety
                   improvements of Llama 2-Chat in order to enable the
                   community to build on our work and contribute to the
                   responsible development of LLMs.",
  month         =  jul,
  year          =  2023,
  url           = "http://arxiv.org/abs/2307.09288",
  archivePrefix = "arXiv",
  eprint        = "2307.09288",
  primaryClass  = "cs.CL",
  arxivid       = "2307.09288",
  doi           = "10.48550/arXiv.2307.09288"
}

@TECHREPORT{Anthropic2024-ca,
  title       = "Introducing the next generation of Claude",
  author      = "{Anthropic}",
  abstract    = "Today, we're announcing the Claude 3 model family, which sets
                 new industry benchmarks across a wide range of cognitive
                 tasks. The family includes three state-of-the-art models in
                 ascending order of capability: Claude 3 Haiku, Claude 3
                 Sonnet, and Claude 3 Opus.",
  institution = "Anthropic",
  month       =  mar,
  year        =  2024,
  url         = "https://www.anthropic.com/news/claude-3-family",
  language    = "en"
}

@ARTICLE{Gemini_Team2023-vq,
  title         = "Gemini: A Family of Highly Capable Multimodal Models",
  author        = "{Gemini Team} ",
  abstract      = "This report introduces a new family of multimodal models,
                   Gemini, that exhibit remarkable capabilities across image,
                   audio, video, and text understanding. The Gemini family
                   consists of Ultra, Pro, and Nano sizes, suitable for
                   applications ranging from complex reasoning tasks to
                   on-device memory-constrained use-cases. Evaluation on a
                   broad range of benchmarks shows that our most-capable Gemini
                   Ultra model advances the state of the art in 30 of 32 of
                   these benchmarks - notably being the first model to achieve
                   human-expert performance on the well-studied exam benchmark
                   MMLU, and improving the state of the art in every one of the
                   20 multimodal benchmarks we examined. We believe that the
                   new capabilities of the Gemini family in cross-modal
                   reasoning and language understanding will enable a wide
                   variety of use cases. We discuss our approach toward
                   post-training and deploying Gemini models responsibly to
                   users through services including Gemini, Gemini Advanced,
                   Google AI Studio, and Cloud Vertex AI.",
  month         =  dec,
  year          =  2023,
  url           = "http://arxiv.org/abs/2312.11805",
  archivePrefix = "arXiv",
  eprint        = "2312.11805",
  primaryClass  = "cs.CL",
  arxivid       = "2312.11805",
  doi           = "10.48550/arXiv.2312.11805"
}

@ARTICLE{OpenAI2023-zj,
  title         = "{GPT-4} Technical Report",
  author        = "{OpenAI} and Achiam, Josh and Adler, Steven and Agarwal,
                   Sandhini and Ahmad, Lama and Akkaya, Ilge and Aleman,
                   Florencia Leoni and Almeida, Diogo and Altenschmidt, Janko
                   and Altman, Sam and Anadkat, Shyamal and Avila, Red and
                   Babuschkin, Igor and Balaji, Suchir and Balcom, Valerie and
                   Baltescu, Paul and Bao, Haiming and Bavarian, Mohammad and
                   Belgum, Jeff and Bello, Irwan and Berdine, Jake and
                   Bernadett-Shapiro, Gabriel and Berner, Christopher and
                   Bogdonoff, Lenny and Boiko, Oleg and Boyd, Madelaine and
                   Brakman, Anna-Luisa and Brockman, Greg and Brooks, Tim and
                   Brundage, Miles and Button, Kevin and Cai, Trevor and
                   Campbell, Rosie and Cann, Andrew and Carey, Brittany and
                   Carlson, Chelsea and Carmichael, Rory and Chan, Brooke and
                   Chang, Che and Chantzis, Fotis and Chen, Derek and Chen,
                   Sully and Chen, Ruby and Chen, Jason and Chen, Mark and
                   Chess, Ben and Cho, Chester and Chu, Casey and Chung, Hyung
                   Won and Cummings, Dave and Currier, Jeremiah and Dai,
                   Yunxing and Decareaux, Cory and Degry, Thomas and Deutsch,
                   Noah and Deville, Damien and Dhar, Arka and Dohan, David and
                   Dowling, Steve and Dunning, Sheila and Ecoffet, Adrien and
                   Eleti, Atty and Eloundou, Tyna and Farhi, David and Fedus,
                   Liam and Felix, Niko and Fishman, Sim{\'o}n Posada and
                   Forte, Juston and Fulford, Isabella and Gao, Leo and
                   Georges, Elie and Gibson, Christian and Goel, Vik and
                   Gogineni, Tarun and Goh, Gabriel and Gontijo-Lopes, Rapha
                   and Gordon, Jonathan and Grafstein, Morgan and Gray, Scott
                   and Greene, Ryan and Gross, Joshua and Gu, Shixiang Shane
                   and Guo, Yufei and Hallacy, Chris and Han, Jesse and Harris,
                   Jeff and He, Yuchen and Heaton, Mike and Heidecke, Johannes
                   and Hesse, Chris and Hickey, Alan and Hickey, Wade and
                   Hoeschele, Peter and Houghton, Brandon and Hsu, Kenny and
                   Hu, Shengli and Hu, Xin and Huizinga, Joost and Jain,
                   Shantanu and Jain, Shawn and Jang, Joanne and Jiang, Angela
                   and Jiang, Roger and Jin, Haozhun and Jin, Denny and Jomoto,
                   Shino and Jonn, Billie and Jun, Heewoo and Kaftan, Tomer and
                   Kaiser, {\L}ukasz and Kamali, Ali and Kanitscheider, Ingmar
                   and Keskar, Nitish Shirish and Khan, Tabarak and Kilpatrick,
                   Logan and Kim, Jong Wook and Kim, Christina and Kim, Yongjik
                   and Kirchner, Jan Hendrik and Kiros, Jamie and Knight, Matt
                   and Kokotajlo, Daniel and Kondraciuk, {\L}ukasz and
                   Kondrich, Andrew and Konstantinidis, Aris and Kosic, Kyle
                   and Krueger, Gretchen and Kuo, Vishal and Lampe, Michael and
                   Lan, Ikai and Lee, Teddy and Leike, Jan and Leung, Jade and
                   Levy, Daniel and Li, Chak Ming and Lim, Rachel and Lin,
                   Molly and Lin, Stephanie and Litwin, Mateusz and Lopez,
                   Theresa and Lowe, Ryan and Lue, Patricia and Makanju, Anna
                   and Malfacini, Kim and Manning, Sam and Markov, Todor and
                   Markovski, Yaniv and Martin, Bianca and Mayer, Katie and
                   Mayne, Andrew and McGrew, Bob and McKinney, Scott Mayer and
                   McLeavey, Christine and McMillan, Paul and McNeil, Jake and
                   Medina, David and Mehta, Aalok and Menick, Jacob and Metz,
                   Luke and Mishchenko, Andrey and Mishkin, Pamela and Monaco,
                   Vinnie and Morikawa, Evan and Mossing, Daniel and Mu, Tong
                   and Murati, Mira and Murk, Oleg and M{\'e}ly, David and
                   Nair, Ashvin and Nakano, Reiichiro and Nayak, Rajeev and
                   Neelakantan, Arvind and Ngo, Richard and Noh, Hyeonwoo and
                   Ouyang, Long and O'Keefe, Cullen and Pachocki, Jakub and
                   Paino, Alex and Palermo, Joe and Pantuliano, Ashley and
                   Parascandolo, Giambattista and Parish, Joel and Parparita,
                   Emy and Passos, Alex and Pavlov, Mikhail and Peng, Andrew
                   and Perelman, Adam and de Avila Belbute Peres, Filipe and
                   Petrov, Michael and de Oliveira Pinto, Henrique Ponde and
                   {Michael} and {Pokorny} and Pokrass, Michelle and Pong,
                   Vitchyr H and Powell, Tolly and Power, Alethea and Power,
                   Boris and Proehl, Elizabeth and Puri, Raul and Radford, Alec
                   and Rae, Jack and Ramesh, Aditya and Raymond, Cameron and
                   Real, Francis and Rimbach, Kendra and Ross, Carl and
                   Rotsted, Bob and Roussez, Henri and Ryder, Nick and
                   Saltarelli, Mario and Sanders, Ted and Santurkar, Shibani
                   and Sastry, Girish and Schmidt, Heather and Schnurr, David
                   and Schulman, John and Selsam, Daniel and Sheppard, Kyla and
                   Sherbakov, Toki and Shieh, Jessica and Shoker, Sarah and
                   Shyam, Pranav and Sidor, Szymon and Sigler, Eric and Simens,
                   Maddie and Sitkin, Jordan and Slama, Katarina and Sohl, Ian
                   and Sokolowsky, Benjamin and Song, Yang and Staudacher,
                   Natalie and Such, Felipe Petroski and Summers, Natalie and
                   Sutskever, Ilya and Tang, Jie and Tezak, Nikolas and
                   Thompson, Madeleine B and Tillet, Phil and Tootoonchian,
                   Amin and Tseng, Elizabeth and Tuggle, Preston and Turley,
                   Nick and Tworek, Jerry and Uribe, Juan Felipe Cer{\'o}n and
                   Vallone, Andrea and Vijayvergiya, Arun and Voss, Chelsea and
                   Wainwright, Carroll and Wang, Justin Jay and Wang, Alvin and
                   Wang, Ben and Ward, Jonathan and Wei, Jason and Weinmann, C
                   J and Welihinda, Akila and Welinder, Peter and Weng, Jiayi
                   and Weng, Lilian and Wiethoff, Matt and Willner, Dave and
                   Winter, Clemens and Wolrich, Samuel and Wong, Hannah and
                   Workman, Lauren and Wu, Sherwin and Wu, Jeff and Wu, Michael
                   and Xiao, Kai and Xu, Tao and Yoo, Sarah and Yu, Kevin and
                   Yuan, Qiming and Zaremba, Wojciech and Zellers, Rowan and
                   Zhang, Chong and Zhang, Marvin and Zhao, Shengjia and Zheng,
                   Tianhao and Zhuang, Juntang and Zhuk, William and Zoph,
                   Barret",
  abstract      = "We report the development of GPT-4, a large-scale,
                   multimodal model which can accept image and text inputs and
                   produce text outputs. While less capable than humans in many
                   real-world scenarios, GPT-4 exhibits human-level performance
                   on various professional and academic benchmarks, including
                   passing a simulated bar exam with a score around the top
                   10\% of test takers. GPT-4 is a Transformer-based model
                   pre-trained to predict the next token in a document. The
                   post-training alignment process results in improved
                   performance on measures of factuality and adherence to
                   desired behavior. A core component of this project was
                   developing infrastructure and optimization methods that
                   behave predictably across a wide range of scales. This
                   allowed us to accurately predict some aspects of GPT-4's
                   performance based on models trained with no more than
                   1/1,000th the compute of GPT-4.",
  month         =  mar,
  year          =  2023,
  url           = "http://arxiv.org/abs/2303.08774",
  archivePrefix = "arXiv",
  eprint        = "2303.08774",
  primaryClass  = "cs.CL",
  arxivid       = "2303.08774",
  doi           = "10.48550/arXiv.2303.08774"
}

@INCOLLECTION{Rodriguez2024-oj,
  title     = "Malicious Uses",
  booktitle = "The Ethics of Advanced {AI} Assistants",
  author    = "Rodriguez, Mikel and Trask, Andrew and Bolina, Vijay and
               Keeling, Geoff and Gabriel, Iason",
  editor    = "Gabriel, Iason and Manzini, Arianna and Keeling, Geoff and
               Hendricks, Lisa Anne and Rieser, Verena and Iqbal, Hasan and
               Toma{\v s}ev, Nenad and Ktena, Ira and Kenton, Zachary and
               Rodriguez, Mikel and El-Sayed, Seliem and Brown, Sasha and
               Akbulut, Canfer and Trask, Andrew and Hughes, Edward and Stevie
               Bergman, A and Shelby, Renee and Marchal, Nahema and Griffin,
               Conor and Mateos-Garcia, Juan and Weidinger, Laura and Street,
               Winnie and Lange, Benjamin and Ingerman, Alex and Lentz, Alison
               and Enger, Reed and Barakat, Andrew and Krakovna, Victoria and
               Siy, John Oliver and Kurth-Nelson, Zeb and McCroskery, Amanda
               and Bolina, Vijay and Law, Harry and Shanahan, Murray and
               Alberts, Lize and Balle, Borja and de Haas, Sarah and Ibitoye,
               Yetunde and Dafoe, Allan and Goldberg, Beth and Krier,
               S{\'e}bastien and Reese, Alexander and Witherspoon, Sims and
               Hawkins, Will and Rauh, Maribeth and Wallace, Don and Franklin,
               Matija and Goldstein, Josh A and Lehman, Joel and Klenk, Michael
               and Vallor, Shannon and Biles, Courtney and Morris, Meredith
               Ringel and King, Helen and Ag{\"u}era y Arcas, Blaise and Isaac,
               William and Manyika, James",
  abstract  = "This paper focuses on the opportunities and the ethical and
               societal risks posed by advanced AI assistants. We define
               advanced AI assistants as artificial agents with natural
               language interfaces, whose function is to plan and execute
               sequences of actions on behalf of a user, across one or more
               domains, in line with the user's expectations. The paper starts
               by considering the technology itself, providing an overview of
               AI assistants, their technical foundations and potential range
               of applications. It then explores questions around AI value
               alignment, well-being, safety and malicious uses. Extending the
               circle of inquiry further, we next consider the relationship
               between advanced AI assistants and individual users in more
               detail, exploring topics such as manipulation and persuasion,
               anthropomorphism, appropriate relationships, trust and privacy.
               With this analysis in place, we consider the deployment of
               advanced assistants at a societal scale, focusing on
               cooperation, equity and access, misinformation, economic impact,
               the environment and how best to evaluate advanced AI assistants.
               Finally, we conclude by providing a range of recommendations for
               researchers, developers, policymakers and public stakeholders.",
  month     =  apr,
  year      =  2024,
  url       = "http://arxiv.org/abs/2404.16244",
  doi       = "10.48550/arXiv.2404.16244"
}

@TECHREPORT{Brooks2024-tu,
  title       = "Video generation models as world simulators",
  author      = "Brooks, Tim and Peebles, Bill and Holmes, Connor and DePue,
                 Will and Guo, Yufei and Jing, Li and Schnurr, David and
                 Taylor, Joe and Luhman, Troy and Luhman, Eric and Ng, Clarence
                 and Wang, Ricky and Ramesh, Aditya",
  institution = "OpenAI",
  month       =  feb,
  year        =  2024,
  url         = "https://openai.com/research/video-generation-models-as-world-simulators"
}

@ARTICLE{Huang2022-nr,
  title         = "Towards Reasoning in Large Language Models: A Survey",
  author        = "Huang, Jie and Chang, Kevin Chen-Chuan",
  abstract      = "Reasoning is a fundamental aspect of human intelligence that
                   plays a crucial role in activities such as problem solving,
                   decision making, and critical thinking. In recent years,
                   large language models (LLMs) have made significant progress
                   in natural language processing, and there is observation
                   that these models may exhibit reasoning abilities when they
                   are sufficiently large. However, it is not yet clear to what
                   extent LLMs are capable of reasoning. This paper provides a
                   comprehensive overview of the current state of knowledge on
                   reasoning in LLMs, including techniques for improving and
                   eliciting reasoning in these models, methods and benchmarks
                   for evaluating reasoning abilities, findings and
                   implications of previous research in this field, and
                   suggestions on future directions. Our aim is to provide a
                   detailed and up-to-date review of this topic and stimulate
                   meaningful discussion and future work.",
  month         =  dec,
  year          =  2022,
  url           = "http://arxiv.org/abs/2212.10403",
  archivePrefix = "arXiv",
  eprint        = "2212.10403",
  primaryClass  = "cs.CL",
  arxivid       = "2212.10403",
  doi           = "10.48550/arXiv.2212.10403"
}

@ARTICLE{Yim2024-cu,
  title    = "Preliminary Evidence of the Use of Generative {AI} in Health Care
              Clinical Services: Systematic Narrative Review",
  author   = "Yim, Dobin and Khuntia, Jiban and Parameswaran, Vijaya and
              Meyers, Arlen",
  abstract = "BACKGROUND: Generative artificial intelligence tools and
              applications (GenAI) are being increasingly used in health care.
              Physicians, specialists, and other providers have started
              primarily using GenAI as an aid or tool to gather knowledge,
              provide information, train, or generate suggestive dialogue
              between physicians and patients or between physicians and
              patients' families or friends. However, unless the use of GenAI
              is oriented to be helpful in clinical service encounters that can
              improve the accuracy of diagnosis, treatment, and patient
              outcomes, the expected potential will not be achieved. As
              adoption continues, it is essential to validate the effectiveness
              of the infusion of GenAI as an intelligent technology in service
              encounters to understand the gap in actual clinical service use
              of GenAI. OBJECTIVE: This study synthesizes preliminary evidence
              on how GenAI assists, guides, and automates clinical service
              rendering and encounters in health care The review scope was
              limited to articles published in peer-reviewed medical journals.
              METHODS: We screened and selected 0.38\% (161/42,459) of articles
              published between January 1, 2020, and May 31, 2023, identified
              from PubMed. We followed the protocols outlined in the PRISMA
              (Preferred Reporting Items for Systematic Reviews and
              Meta-Analyses) guidelines to select highly relevant studies with
              at least 1 element on clinical use, evaluation, and validation to
              provide evidence of GenAI use in clinical services. The articles
              were classified based on their relevance to clinical service
              functions or activities using the descriptive and analytical
              information presented in the articles. RESULTS: Of 161 articles,
              141 (87.6\%) reported using GenAI to assist services through
              knowledge access, collation, and filtering. GenAI was used for
              disease detection (19/161, 11.8\%), diagnosis (14/161, 8.7\%),
              and screening processes (12/161, 7.5\%) in the areas of radiology
              (17/161, 10.6\%), cardiology (12/161, 7.5\%), gastrointestinal
              medicine (4/161, 2.5\%), and diabetes (6/161, 3.7\%). The
              literature synthesis in this study suggests that GenAI is mainly
              used for diagnostic processes, improvement of diagnosis accuracy,
              and screening and diagnostic purposes using knowledge access.
              Although this solves the problem of knowledge access and may
              improve diagnostic accuracy, it is oriented toward higher value
              creation in health care. CONCLUSIONS: GenAI informs rather than
              assisting or automating clinical service functions in health
              care. There is potential in clinical service, but it has yet to
              be actualized for GenAI. More clinical service-level evidence
              that GenAI is used to streamline some functions or provides more
              automated help than only information retrieval is needed. To
              transform health care as purported, more studies related to GenAI
              applications must automate and guide human-performed services and
              keep up with the optimism that forward-thinking health care
              organizations will take advantage of GenAI.",
  journal  = "JMIR Med Inform",
  volume   =  12,
  pages    = "e52073",
  month    =  mar,
  year     =  2024,
  url      = "http://doi.org/10.2196/52073",
  keywords = "GenAI; clinical; digital; generative artificial intelligence
              tools and applications; health care; service; transformation",
  language = "en",
  issn     = "2291-9694",
  pmid     = "38506918",
  doi      = "10.2196/52073",
  pmc      = "PMC10993141"
}

@ARTICLE{Yang2023-kv,
  title         = "{BigTranslate}: Augmenting Large Language Models with
                   Multilingual Translation Capability over 100 Languages",
  author        = "Yang, Wen and Li, Chong and Zhang, Jiajun and Zong,
                   Chengqing",
  abstract      = "Large language models (LLMs) demonstrate promising
                   translation performance among various natural languages.
                   However, many LLMs especially the open-sourced ones, such as
                   BLOOM and LLaMA, are English-dominant and support only
                   dozens of natural languages, making the potential of LLMs on
                   language translation less explored. In this work, we present
                   BigTranslate which adapts LLaMA that covers only 20
                   languages and enhances it with multilingual translation
                   capability on more than 100 languages. BigTranslate is built
                   upon LLaMA-13B and it is optimized in three steps. First, we
                   continue training LLaMA with massive Chinese monolingual
                   data. Second, we continue training the model with a
                   large-scale parallel dataset that covers 102 natural
                   languages. Third, we instruct-tune the foundation model with
                   multilingual translation instructions, leading to our
                   BigTranslate model. The preliminary experiments on
                   multilingual translation show that BigTranslate performs
                   comparably with ChatGPT and Google Translate in many
                   languages and even outperforms ChatGPT in 8 language pairs.
                   We release the BigTranslate model and hope it can advance
                   the research progress.",
  month         =  may,
  year          =  2023,
  url           = "http://arxiv.org/abs/2305.18098",
  archivePrefix = "arXiv",
  eprint        = "2305.18098",
  primaryClass  = "cs.CL",
  arxivid       = "2305.18098",
  doi           = "10.48550/arXiv.2305.18098"
}

@ARTICLE{Wang2023-vr,
  title         = "{In-Context} Learning Unlocked for Diffusion Models",
  author        = "Wang, Zhendong and Jiang, Yifan and Lu, Yadong and Shen,
                   Yelong and He, Pengcheng and Chen, Weizhu and Wang,
                   Zhangyang and Zhou, Mingyuan",
  abstract      = "We present Prompt Diffusion, a framework for enabling
                   in-context learning in diffusion-based generative models.
                   Given a pair of task-specific example images, such as depth
                   from/to image and scribble from/to image, and a text
                   guidance, our model automatically understands the underlying
                   task and performs the same task on a new query image
                   following the text guidance. To achieve this, we propose a
                   vision-language prompt that can model a wide range of
                   vision-language tasks and a diffusion model that takes it as
                   input. The diffusion model is trained jointly over six
                   different tasks using these prompts. The resulting Prompt
                   Diffusion model is the first diffusion-based vision-language
                   foundation model capable of in-context learning. It
                   demonstrates high-quality in-context generation on the
                   trained tasks and generalizes effectively to new, unseen
                   vision tasks with their respective prompts. Our model also
                   shows compelling text-guided image editing results. Our
                   framework aims to facilitate research into in-context
                   learning for computer vision. We share our code and
                   pre-trained models at
                   https://github.com/Zhendong-Wang/Prompt-Diffusion.",
  month         =  may,
  year          =  2023,
  url           = "http://arxiv.org/abs/2305.01115",
  archivePrefix = "arXiv",
  eprint        = "2305.01115",
  primaryClass  = "cs.CV",
  arxivid       = "2305.01115",
  doi           = "10.48550/arXiv.2305.01115"
}

@ARTICLE{Wallace2024-in,
  title         = "The Instruction Hierarchy: Training {LLMs} to Prioritize
                   Privileged Instructions",
  author        = "Wallace, Eric and Xiao, Kai and Leike, Reimar and Weng,
                   Lilian and Heidecke, Johannes and Beutel, Alex",
  abstract      = "Today's LLMs are susceptible to prompt injections,
                   jailbreaks, and other attacks that allow adversaries to
                   overwrite a model's original instructions with their own
                   malicious prompts. In this work, we argue that one of the
                   primary vulnerabilities underlying these attacks is that
                   LLMs often consider system prompts (e.g., text from an
                   application developer) to be the same priority as text from
                   untrusted users and third parties. To address this, we
                   propose an instruction hierarchy that explicitly defines how
                   models should behave when instructions of different
                   priorities conflict. We then propose a data generation
                   method to demonstrate this hierarchical instruction
                   following behavior, which teaches LLMs to selectively ignore
                   lower-privileged instructions. We apply this method to
                   GPT-3.5, showing that it drastically increases robustness --
                   even for attack types not seen during training -- while
                   imposing minimal degradations on standard capabilities.",
  month         =  apr,
  year          =  2024,
  url           = "http://arxiv.org/abs/2404.13208",
  archivePrefix = "arXiv",
  eprint        = "2404.13208",
  primaryClass  = "cs.CR",
  arxivid       = "2404.13208",
  doi           = "10.48550/arXiv.2404.13208"
}

@ARTICLE{Wallace2019-tx,
  title         = "Universal Adversarial Triggers for Attacking and Analyzing
                   {NLP}",
  author        = "Wallace, Eric and Feng, Shi and Kandpal, Nikhil and Gardner,
                   Matt and Singh, Sameer",
  abstract      = "Adversarial examples highlight model vulnerabilities and are
                   useful for evaluation and interpretation. We define
                   universal adversarial triggers: input-agnostic sequences of
                   tokens that trigger a model to produce a specific prediction
                   when concatenated to any input from a dataset. We propose a
                   gradient-guided search over tokens which finds short trigger
                   sequences (e.g., one word for classification and four words
                   for language modeling) that successfully trigger the target
                   prediction. For example, triggers cause SNLI entailment
                   accuracy to drop from 89.94\% to 0.55\%, 72\% of ``why''
                   questions in SQuAD to be answered ``to kill american
                   people'', and the GPT-2 language model to spew racist output
                   even when conditioned on non-racial contexts. Furthermore,
                   although the triggers are optimized using white-box access
                   to a specific model, they transfer to other models for all
                   tasks we consider. Finally, since triggers are
                   input-agnostic, they provide an analysis of global model
                   behavior. For instance, they confirm that SNLI models
                   exploit dataset biases and help to diagnose heuristics
                   learned by reading comprehension models.",
  month         =  aug,
  year          =  2019,
  url           = "http://arxiv.org/abs/1908.07125",
  archivePrefix = "arXiv",
  eprint        = "1908.07125",
  primaryClass  = "cs.CL",
  arxivid       = "1908.07125",
  doi           = "10.48550/arXiv.1908.07125"
}

@ARTICLE{Vaccari2020-uo,
  title     = "Deepfakes and Disinformation: Exploring the Impact of Synthetic
               Political Video on Deception, Uncertainty, and Trust in News",
  author    = "Vaccari, Cristian and Chadwick, Andrew",
  abstract  = "Artificial Intelligence (AI) now enables the mass creation of
               what have become known as ?deepfakes?: synthetic videos that
               closely resemble real videos. Integrating theories about the
               power of visual communication and the role played by uncertainty
               in undermining trust in public discourse, we explain the likely
               contribution of deepfakes to online disinformation.
               Administering novel experimental treatments to a large
               representative sample of the United Kingdom population allowed
               us to compare people?s evaluations of deepfakes. We find that
               people are more likely to feel uncertain than to be misled by
               deepfakes, but this resulting uncertainty, in turn, reduces
               trust in news on social media. We conclude that deepfakes may
               contribute toward generalized indeterminacy and cynicism,
               further intensifying recent challenges to online civic culture
               in democratic societies.",
  journal   = "Social Media + Society",
  publisher = "SAGE Publications Ltd",
  volume    =  6,
  number    =  1,
  pages     = "2056305120903408",
  month     =  jan,
  year      =  2020,
  url       = "https://doi.org/10.1177/2056305120903408",
  issn      = "2056-3051",
  doi       = "10.1177/2056305120903408"
}

@ARTICLE{Tian2023-nf,
  title         = "Is {ChatGPT} the Ultimate Programming Assistant -- How far
                   is it?",
  author        = "Tian, Haoye and Lu, Weiqi and Li, Tsz On and Tang, Xunzhu
                   and Cheung, Shing-Chi and Klein, Jacques and Bissyand{\'e},
                   Tegawend{\'e} F",
  abstract      = "Recently, the ChatGPT LLM has received great attention: it
                   can be used as a bot for discussing source code, prompting
                   it to suggest changes, provide descriptions or even generate
                   code. Typical demonstrations generally focus on existing
                   benchmarks, which may have been used in model training
                   (i.e., data leakage). To assess the feasibility of using an
                   LLM as a useful assistant bot for programmers, we must
                   assess its realistic capabilities on unseen problems as well
                   as its capabilities on various tasks. In this paper, we
                   present an empirical study of ChatGPT's potential as a fully
                   automated programming assistant, focusing on the tasks of
                   code generation, program repair, and code summariziation.
                   The study investigates ChatGPT's performance on common
                   programming problems and compares it with state-of-the-art
                   approaches on two benchmarks. Among several findings, our
                   study shows that ChatGPT is effective in dealing with common
                   programming problems. However, our experiments also reveal
                   limitations in terms of its attention span: detailed
                   descriptions will constrain the focus of ChatGPT and prevent
                   it from leveraging its vast knowledge to solve the actual
                   problem. Surprisingly, we have identified the ability of
                   ChatGPT to reason the original intention of the code. We
                   expect future work to build on this insight for dealing with
                   the open question of the oracle problem. Our findings
                   contribute interesting insights to the development of LLMs
                   for programming assistance, notably by demonstrating the
                   importance of prompt engineering, and providing a better
                   understanding of ChatGPT's practical applications for
                   software engineering.",
  month         =  apr,
  year          =  2023,
  url           = "http://arxiv.org/abs/2304.11938",
  archivePrefix = "arXiv",
  eprint        = "2304.11938",
  primaryClass  = "cs.SE",
  arxivid       = "2304.11938",
  doi           = "10.48550/arXiv.2304.11938"
}

@ARTICLE{Syed2020-na,
  title    = "Adapting Language Models for {Non-Parallel} {Author-Stylized}
              Rewriting",
  author   = "Syed, Bakhtiyar and Verma, Gaurav and Srinivasan, Balaji Vasan
              and Natarajan, Anandhavelu and Varma, Vasudeva",
  abstract = "Given the recent progress in language modeling using
              Transformer-based neural models and an active interest in
              generating stylized text, we present an approach to leverage the
              generalization capabilities of a language model to rewrite an
              input text in a target author's style. Our proposed approach
              adapts a pre-trained language model to generate author-stylized
              text by fine-tuning on the author-specific corpus using a
              denoising autoencoder (DAE) loss in a cascaded encoder-decoder
              framework. Optimizing over DAE loss allows our model to learn the
              nuances of an author's style without relying on parallel data,
              which has been a severe limitation of the previous related works
              in this space. To evaluate the efficacy of our approach, we
              propose a linguistically-motivated framework to quantify
              stylistic alignment of the generated text to the target author at
              lexical, syntactic and surface levels. The evaluation framework
              is both interpretable as it leads to several insights about the
              model, and self-contained as it does not rely on external
              classifiers, e.g. sentiment or formality classifiers. Qualitative
              and quantitative assessment indicates that the proposed approach
              rewrites the input text with better alignment to the target style
              while preserving the original content better than
              state-of-the-art baselines.",
  journal  = "AAAI",
  volume   =  34,
  number   =  05,
  pages    = "9008--9015",
  month    =  apr,
  year     =  2020,
  url      = "https://ojs.aaai.org/index.php/AAAI/article/view/6433",
  language = "en",
  issn     = "2374-3468, 2374-3468",
  doi      = "10.1609/aaai.v34i05.6433"
}

@INCOLLECTION{Sundar2008-qc,
  title     = "The {MAIN} model: A heuristic approach to understanding
               technology effects on credibility",
  booktitle = "Digital Media, Youth, and Credibility",
  author    = "Sundar, S S",
  editor    = "Metzger, Miriam J and Flanagin, Andrew J",
  abstract  = "The difficulties in determining the quality of information on
               the Internet--in particular, the implications of wide access and
               questionable credibility for youth and learning.Today we have
               access to an almost inconceivably vast amount of information,
               from sources that are increasingly portable, accessible, and
               interactive. The Internet and the explosion of digital media
               content have made more information available from more sources
               to more people than at any other time in human history. This
               brings an infinite number of opportunities for learning, social
               connection, and entertainment. But at the same time, the origin
               of information, its quality, and its veracity are often
               difficult to assess. This volume addresses the issue of
               credibility--the objective and subjective components that make
               information believable--in the contemporary media environment.
               The contributors look particularly at youth audiences and
               experiences, considering the implications of wide access and the
               questionable credibility of information for youth and learning.
               They discuss such topics as the credibility of health
               information online, how to teach credibility assessment, and
               public policy solutions. Much research has been done on
               credibility and new media, but little of it focuses on users
               younger than college students. Digital Media, Youth, and
               Credibility fills this gap in the literature.ContributorsMatthew
               S. Eastin, Gunther Eysenbach, Brian Hilligoss, Frances Jacobson
               Harris, R. David Lankes, Soo Young Rieh, S. Shyam Sundar, Fred
               W. Weingarten",
  publisher = "MIT Press",
  pages     = "73--100",
  year      =  2008,
  url       = "https://library.oapen.org/handle/20.500.12657/26088",
  language  = "en",
  isbn      = "9780262062732"
}

@ARTICLE{Shevlane2022-lk,
  title         = "Structured access: an emerging paradigm for safe {AI}
                   deployment",
  author        = "Shevlane, Toby",
  abstract      = "Structured access is an emerging paradigm for the safe
                   deployment of artificial intelligence (AI). Instead of
                   openly disseminating AI systems, developers facilitate
                   controlled, arm's length interactions with their AI systems.
                   The aim is to prevent dangerous AI capabilities from being
                   widely accessible, whilst preserving access to AI
                   capabilities that can be used safely. The developer must
                   both restrict how the AI system can be used, and prevent the
                   user from circumventing these restrictions through
                   modification or reverse engineering of the AI system.
                   Structured access is most effective when implemented through
                   cloud-based AI services, rather than disseminating AI
                   software that runs locally on users' hardware. Cloud-based
                   interfaces provide the AI developer greater scope for
                   controlling how the AI system is used, and for protecting
                   against unauthorized modifications to the system's design.
                   This chapter expands the discussion of ``publication norms''
                   in the AI community, which to date has focused on the
                   question of how the informational content of AI research
                   projects should be disseminated (e.g., code and models).
                   Although this is an important question, there are limits to
                   what can be achieved through the control of information
                   flows. Structured access views AI software not only as
                   information that can be shared but also as a tool with which
                   users can have arm's length interactions. There are early
                   examples of structured access being practiced by AI
                   developers, but there is much room for further development,
                   both in the functionality of cloud-based interfaces and in
                   the wider institutional framework.",
  month         =  jan,
  year          =  2022,
  url           = "http://arxiv.org/abs/2201.05159",
  archivePrefix = "arXiv",
  eprint        = "2201.05159",
  primaryClass  = "cs.AI",
  arxivid       = "2201.05159",
  doi           = "10.48550/arXiv.2201.05159"
}

@ARTICLE{Shevlane2023-av,
  title         = "Model evaluation for extreme risks",
  author        = "Shevlane, Toby and Farquhar, Sebastian and Garfinkel, Ben
                   and Phuong, Mary and Whittlestone, Jess and Leung, Jade and
                   Kokotajlo, Daniel and Marchal, Nahema and Anderljung, Markus
                   and Kolt, Noam and Ho, Lewis and Siddarth, Divya and Avin,
                   Shahar and Hawkins, Will and Kim, Been and Gabriel, Iason
                   and Bolina, Vijay and Clark, Jack and Bengio, Yoshua and
                   Christiano, Paul and Dafoe, Allan",
  abstract      = "Current approaches to building general-purpose AI systems
                   tend to produce systems with both beneficial and harmful
                   capabilities. Further progress in AI development could lead
                   to capabilities that pose extreme risks, such as offensive
                   cyber capabilities or strong manipulation skills. We explain
                   why model evaluation is critical for addressing extreme
                   risks. Developers must be able to identify dangerous
                   capabilities (through ``dangerous capability evaluations'')
                   and the propensity of models to apply their capabilities for
                   harm (through ``alignment evaluations''). These evaluations
                   will become critical for keeping policymakers and other
                   stakeholders informed, and for making responsible decisions
                   about model training, deployment, and security.",
  month         =  may,
  year          =  2023,
  url           = "http://arxiv.org/abs/2305.15324",
  archivePrefix = "arXiv",
  eprint        = "2305.15324",
  primaryClass  = "cs.AI",
  arxivid       = "2305.15324",
  doi           = "10.48550/arXiv.2305.15324"
}

@ARTICLE{Shen2023-mt,
  title         = "``Do Anything Now'': Characterizing and Evaluating
                   {In-The-Wild} Jailbreak Prompts on Large Language Models",
  author        = "Shen, Xinyue and Chen, Zeyuan and Backes, Michael and Shen,
                   Yun and Zhang, Yang",
  abstract      = "The misuse of large language models (LLMs) has drawn
                   significant attention from the general public and LLM
                   vendors. One particular type of adversarial prompt, known as
                   jailbreak prompt, has emerged as the main attack vector to
                   bypass the safeguards and elicit harmful content from LLMs.
                   In this paper, employing our new framework JailbreakHub, we
                   conduct a comprehensive analysis of 1,405 jailbreak prompts
                   spanning from December 2022 to December 2023. We identify
                   131 jailbreak communities and discover unique
                   characteristics of jailbreak prompts and their major attack
                   strategies, such as prompt injection and privilege
                   escalation. We also observe that jailbreak prompts
                   increasingly shift from online Web communities to
                   prompt-aggregation websites and 28 user accounts have
                   consistently optimized jailbreak prompts over 100 days. To
                   assess the potential harm caused by jailbreak prompts, we
                   create a question set comprising 107,250 samples across 13
                   forbidden scenarios. Leveraging this dataset, our
                   experiments on six popular LLMs show that their safeguards
                   cannot adequately defend jailbreak prompts in all scenarios.
                   Particularly, we identify five highly effective jailbreak
                   prompts that achieve 0.95 attack success rates on ChatGPT
                   (GPT-3.5) and GPT-4, and the earliest one has persisted
                   online for over 240 days. We hope that our study can
                   facilitate the research community and LLM vendors in
                   promoting safer and regulated LLMs.",
  month         =  aug,
  year          =  2023,
  url           = "http://arxiv.org/abs/2308.03825",
  archivePrefix = "arXiv",
  eprint        = "2308.03825",
  primaryClass  = "cs.CR",
  arxivid       = "2308.03825",
  doi           = "10.48550/arXiv.2308.03825"
}

@ARTICLE{Schick2023-oo,
  title         = "Toolformer: Language Models Can Teach Themselves to Use
                   Tools",
  author        = "Schick, Timo and Dwivedi-Yu, Jane and Dess{\`\i}, Roberto
                   and Raileanu, Roberta and Lomeli, Maria and Zettlemoyer,
                   Luke and Cancedda, Nicola and Scialom, Thomas",
  abstract      = "Language models (LMs) exhibit remarkable abilities to solve
                   new tasks from just a few examples or textual instructions,
                   especially at scale. They also, paradoxically, struggle with
                   basic functionality, such as arithmetic or factual lookup,
                   where much simpler and smaller models excel. In this paper,
                   we show that LMs can teach themselves to use external tools
                   via simple APIs and achieve the best of both worlds. We
                   introduce Toolformer, a model trained to decide which APIs
                   to call, when to call them, what arguments to pass, and how
                   to best incorporate the results into future token
                   prediction. This is done in a self-supervised way, requiring
                   nothing more than a handful of demonstrations for each API.
                   We incorporate a range of tools, including a calculator, a
                   Q\&A system, two different search engines, a translation
                   system, and a calendar. Toolformer achieves substantially
                   improved zero-shot performance across a variety of
                   downstream tasks, often competitive with much larger models,
                   without sacrificing its core language modeling abilities.",
  month         =  feb,
  year          =  2023,
  url           = "http://arxiv.org/abs/2302.04761",
  archivePrefix = "arXiv",
  eprint        = "2302.04761",
  primaryClass  = "cs.CL",
  arxivid       = "2302.04761",
  doi           = "10.48550/arXiv.2302.04761"
}

@ARTICLE{Roozenbeek2022-vp,
  title    = "Psychological inoculation improves resilience against
              misinformation on social media",
  author   = "Roozenbeek, Jon and van der Linden, Sander and Goldberg, Beth and
              Rathje, Steve and Lewandowsky, Stephan",
  abstract = "Online misinformation continues to have adverse consequences for
              society. Inoculation theory has been put forward as a way to
              reduce susceptibility to misinformation by informing people about
              how they might be misinformed, but its scalability has been
              elusive both at a theoretical level and a practical level. We
              developed five short videos that inoculate people against
              manipulation techniques commonly used in misinformation:
              emotionally manipulative language, incoherence, false
              dichotomies, scapegoating, and ad hominem attacks. In seven
              preregistered studies, i.e., six randomized controlled studies (n
              = 6464) and an ecologically valid field study on YouTube (n =
              22,632), we find that these videos improve manipulation technique
              recognition, boost confidence in spotting these techniques,
              increase people's ability to discern trustworthy from
              untrustworthy content, and improve the quality of their sharing
              decisions. These effects are robust across the political spectrum
              and a wide variety of covariates. We show that psychological
              inoculation campaigns on social media are effective at improving
              misinformation resilience at scale.",
  journal  = "Sci Adv",
  volume   =  8,
  number   =  34,
  pages    = "eabo6254",
  month    =  aug,
  year     =  2022,
  url      = "http://doi.org/10.1126/sciadv.abo6254",
  language = "en",
  issn     = "2375-2548",
  pmid     = "36001675",
  doi      = "10.1126/sciadv.abo6254",
  pmc      = "PMC9401631"
}

@ARTICLE{Gemini_Team2024-ul,
  title         = "Gemini 1.5: Unlocking multimodal understanding across
                   millions of tokens of context",
  author        = "Gemini Team ,2024" ,
  abstract      = "In this report, we present the latest model of the Gemini
                   family, Gemini 1.5 Pro, a highly compute-efficient
                   multimodal mixture-of-experts model capable of recalling and
                   reasoning over fine-grained information from millions of
                   tokens of context, including multiple long documents and
                   hours of video and audio. Gemini 1.5 Pro achieves
                   near-perfect recall on long-context retrieval tasks across
                   modalities, improves the state-of-the-art in long-document
                   QA, long-video QA and long-context ASR, and matches or
                   surpasses Gemini 1.0 Ultra's state-of-the-art performance
                   across a broad set of benchmarks. Studying the limits of
                   Gemini 1.5 Pro's long-context ability, we find continued
                   improvement in next-token prediction and near-perfect
                   retrieval (>99\%) up to at least 10M tokens, a generational
                   leap over existing models such as Claude 2.1 (200k) and
                   GPT-4 Turbo (128k). Finally, we highlight surprising new
                   capabilities of large language models at the frontier; when
                   given a grammar manual for Kalamang, a language with fewer
                   than 200 speakers worldwide, the model learns to translate
                   English to Kalamang at a similar level to a person who
                   learned from the same content.",
  month         =  mar,
  year          =  2024,
  url           = "http://arxiv.org/abs/2403.05530",
  archivePrefix = "arXiv",
  eprint        = "2403.05530",
  primaryClass  = "cs.CL",
  arxivid       = "2403.05530",
  doi           = "10.48550/arXiv.2403.05530"
}

@INPROCEEDINGS{Qadir2023-es,
  title     = "Engineering Education in the Era of {ChatGPT}: Promise and
               Pitfalls of Generative {AI} for Education",
  booktitle = "2023 {IEEE} Global Engineering Education Conference ({EDUCON})",
  author    = "Qadir, Junaid",
  abstract  = "Engineering education is constantly evolving to keep up with the
               latest technological developments and meet the changing needs of
               the engineering industry. One promising development in this
               field is the use of generative artificial intelligence
               technology, such as the ChatGPT conversational agent. ChatGPT
               has the potential to offer personalized and effective learning
               experiences by providing students with customized feedback and
               explanations, as well as creating realistic virtual simulations
               for hands-on learning. However, it is important to also consider
               the limitations of this technology. ChatGPT and other generative
               AI systems are only as good as their training data and may
               perpetuate biases or even generate and spread misinformation.
               Additionally, the use of generative AI in education raises
               ethical concerns such as the potential for unethical or
               dishonest use by students and the potential unemployment of
               humans who are made redundant by technology. While the current
               state of generative AI technology represented by ChatGPT is
               impressive but flawed, it is only a preview of what is to come.
               It is important for engineering educators to understand the
               implications of this technology and study how to adapt the
               engineering education ecosystem to ensure that the next
               generation of engineers can take advantage of the benefits
               offered by generative AI while minimizing any negative
               consequences.",
  publisher = "IEEE",
  pages     = "1--9",
  month     =  may,
  year      =  2023,
  url       = "http://dx.doi.org/10.1109/EDUCON54358.2023.10125121",
  issn      = "2165-9567, 2165-9559",
  doi       = "10.1109/EDUCON54358.2023.10125121"
}

@ARTICLE{Perez2022-cw,
  title         = "Ignore Previous Prompt: Attack Techniques For Language
                   Models",
  author        = "Perez, F{\'a}bio and Ribeiro, Ian",
  abstract      = "Transformer-based large language models (LLMs) provide a
                   powerful foundation for natural language tasks in
                   large-scale customer-facing applications. However, studies
                   that explore their vulnerabilities emerging from malicious
                   user interaction are scarce. By proposing PromptInject, a
                   prosaic alignment framework for mask-based iterative
                   adversarial prompt composition, we examine how GPT-3, the
                   most widely deployed language model in production, can be
                   easily misaligned by simple handcrafted inputs. In
                   particular, we investigate two types of attacks -- goal
                   hijacking and prompt leaking -- and demonstrate that even
                   low-aptitude, but sufficiently ill-intentioned agents, can
                   easily exploit GPT-3's stochastic nature, creating long-tail
                   risks. The code for PromptInject is available at
                   https://github.com/agencyenterprise/PromptInject.",
  month         =  nov,
  year          =  2022,
  url           = "http://arxiv.org/abs/2211.09527",
  archivePrefix = "arXiv",
  eprint        = "2211.09527",
  primaryClass  = "cs.CL",
  arxivid       = "2211.09527",
  doi           = "10.48550/arXiv.2211.09527"
}

@ARTICLE{Nightingale2022-gl,
  title    = "{AI-synthesized} faces are indistinguishable from real faces and
              more trustworthy",
  author   = "Nightingale, Sophie J and Farid, Hany",
  abstract = "Artificial intelligence (AI)-synthesized text, audio, image, and
              video are being weaponized for the purposes of nonconsensual
              intimate imagery, financial fraud, and disinformation campaigns.
              Our evaluation of the photorealism of AI-synthesized faces
              indicates that synthesis engines have passed through the uncanny
              valley and are capable of creating faces that are
              indistinguishable-and more trustworthy-than real faces.",
  journal  = "Proc. Natl. Acad. Sci. U. S. A.",
  volume   =  119,
  number   =  8,
  month    =  feb,
  year     =  2022,
  url      = "http://doi.org/10.1073/pnas.2120481119",
  keywords = "deep fakes; face perception",
  language = "en",
  issn     = "0027-8424, 1091-6490",
  pmid     = "35165187",
  doi      = "10.1073/pnas.2120481119",
  pmc      = "PMC8872790"
}

@INCOLLECTION{Pauly2024-yy,
  title     = "Technology: Disconnecting the Gordian Node",
  booktitle = "Munich Security Report 2024",
  author    = "Pauly, Jintro",
  editor    = "{Tobias Bunde, Sophie Eisentraut, and Leonard Sch{\"u}tte}",
  pages     = "95--101",
  month     =  feb,
  year      =  2024,
  url       = "https://securityconference.org/en/publications/munich-security-report-2024/technology/",
  language  = "en",
  doi       = "10.47342/BMQK9457"
}

@INPROCEEDINGS{Maynez2020-xl,
  title     = "On Faithfulness and Factuality in Abstractive Summarization",
  booktitle = "Proceedings of the 58th Annual Meeting of the Association for
               Computational Linguistics",
  author    = "Maynez, Joshua and Narayan, Shashi and Bohnet, Bernd and
               McDonald, Ryan",
  editor    = "Jurafsky, Dan and Chai, Joyce and Schluter, Natalie and
               Tetreault, Joel",
  abstract  = "It is well known that the standard likelihood training and
               approximate decoding objectives in neural text generation models
               lead to less human-like responses for open-ended tasks such as
               language modeling and story generation. In this paper we have
               analyzed limitations of these models for abstractive document
               summarization and found that these models are highly prone to
               hallucinate content that is unfaithful to the input document. We
               conducted a large scale human evaluation of several neural
               abstractive summarization systems to better understand the types
               of hallucinations they produce. Our human annotators found
               substantial amounts of hallucinated content in all model
               generated summaries. However, our analysis does show that
               pretrained models are better summarizers not only in terms of
               raw metrics, i.e., ROUGE, but also in generating faithful and
               factual summaries as evaluated by humans. Furthermore, we show
               that textual entailment measures better correlate with
               faithfulness than standard metrics, potentially leading the way
               to automatic evaluation metrics as well as training and decoding
               criteria.",
  publisher = "Association for Computational Linguistics",
  pages     = "1906--1919",
  month     =  jul,
  year      =  2020,
  url       = "http://doi.org/10.18653/v1/2020.acl-main.173",
  address   = "Online",
  doi       = "10.18653/v1/2020.acl-main.173"
}

@ARTICLE{Lugmayr2022-tc,
  title         = "{RePaint}: Inpainting using Denoising Diffusion
                   Probabilistic Models",
  author        = "Lugmayr, Andreas and Danelljan, Martin and Romero, Andres
                   and Yu, Fisher and Timofte, Radu and Van Gool, Luc",
  abstract      = "Free-form inpainting is the task of adding new content to an
                   image in the regions specified by an arbitrary binary mask.
                   Most existing approaches train for a certain distribution of
                   masks, which limits their generalization capabilities to
                   unseen mask types. Furthermore, training with pixel-wise and
                   perceptual losses often leads to simple textural extensions
                   towards the missing areas instead of semantically meaningful
                   generation. In this work, we propose RePaint: A Denoising
                   Diffusion Probabilistic Model (DDPM) based inpainting
                   approach that is applicable to even extreme masks. We employ
                   a pretrained unconditional DDPM as the generative prior. To
                   condition the generation process, we only alter the reverse
                   diffusion iterations by sampling the unmasked regions using
                   the given image information. Since this technique does not
                   modify or condition the original DDPM network itself, the
                   model produces high-quality and diverse output images for
                   any inpainting form. We validate our method for both faces
                   and general-purpose image inpainting using standard and
                   extreme masks. RePaint outperforms state-of-the-art
                   Autoregressive, and GAN approaches for at least five out of
                   six mask distributions. Github Repository: git.io/RePaint",
  month         =  jan,
  year          =  2022,
  url           = "http://arxiv.org/abs/2201.09865",
  archivePrefix = "arXiv",
  eprint        = "2201.09865",
  primaryClass  = "cs.CV",
  arxivid       = "2201.09865",
  doi           = "10.48550/arXiv.2201.09865"
}

@ARTICLE{Lin2024-di,
  title         = "Malla: Demystifying Real-world Large Language Model
                   Integrated Malicious Services",
  author        = "Lin, Zilong and Cui, Jian and Liao, Xiaojing and Wang,
                   Xiaofeng",
  abstract      = "The underground exploitation of large language models (LLMs)
                   for malicious services (i.e., Malla) is witnessing an
                   uptick, amplifying the cyber threat landscape and posing
                   questions about the trustworthiness of LLM technologies.
                   However, there has been little effort to understand this new
                   cybercrime, in terms of its magnitude, impact, and
                   techniques. In this paper, we conduct the first systematic
                   study on 212 real-world Mallas, uncovering their
                   proliferation in underground marketplaces and exposing their
                   operational modalities. Our study discloses the Malla
                   ecosystem, revealing its significant growth and impact on
                   today's public LLM services. Through examining 212 Mallas,
                   we uncovered eight backend LLMs used by Mallas, along with
                   182 prompts that circumvent the protective measures of
                   public LLM APIs. We further demystify the tactics employed
                   by Mallas, including the abuse of uncensored LLMs and the
                   exploitation of public LLM APIs through jailbreak prompts.
                   Our findings enable a better understanding of the real-world
                   exploitation of LLMs by cybercriminals, offering insights
                   into strategies to counteract this cybercrime.",
  month         =  jan,
  year          =  2024,
  url           = "http://arxiv.org/abs/2401.03315",
  archivePrefix = "arXiv",
  eprint        = "2401.03315",
  primaryClass  = "cs.CR",
  arxivid       = "2401.03315",
  doi           = "10.48550/arXiv.2401.03315"
}

@ARTICLE{Liu2023-vr,
  title         = "Jailbreaking {ChatGPT} via Prompt Engineering: An Empirical
                   Study",
  author        = "Liu, Yi and Deng, Gelei and Xu, Zhengzi and Li, Yuekang and
                   Zheng, Yaowen and Zhang, Ying and Zhao, Lida and Zhang,
                   Tianwei and Wang, Kailong and Liu, Yang",
  abstract      = "Large Language Models (LLMs), like ChatGPT, have
                   demonstrated vast potential but also introduce challenges
                   related to content constraints and potential misuse. Our
                   study investigates three key research questions: (1) the
                   number of different prompt types that can jailbreak LLMs,
                   (2) the effectiveness of jailbreak prompts in circumventing
                   LLM constraints, and (3) the resilience of ChatGPT against
                   these jailbreak prompts. Initially, we develop a
                   classification model to analyze the distribution of existing
                   prompts, identifying ten distinct patterns and three
                   categories of jailbreak prompts. Subsequently, we assess the
                   jailbreak capability of prompts with ChatGPT versions 3.5
                   and 4.0, utilizing a dataset of 3,120 jailbreak questions
                   across eight prohibited scenarios. Finally, we evaluate the
                   resistance of ChatGPT against jailbreak prompts, finding
                   that the prompts can consistently evade the restrictions in
                   40 use-case scenarios. The study underscores the importance
                   of prompt structures in jailbreaking LLMs and discusses the
                   challenges of robust jailbreak prompt generation and
                   prevention.",
  month         =  may,
  year          =  2023,
  url           = "http://arxiv.org/abs/2305.13860",
  archivePrefix = "arXiv",
  eprint        = "2305.13860",
  primaryClass  = "cs.SE",
  arxivid       = "2305.13860",
  doi           = "10.48550/arXiv.2305.13860"
}

@ARTICLE{Leibowicz2021-va,
  title         = "The Deepfake Detection Dilemma: A Multistakeholder
                   Exploration of Adversarial Dynamics in Synthetic Media",
  author        = "Leibowicz, Claire and McGregor, Sean and Ovadya, Aviv",
  abstract      = "Synthetic media detection technologies label media as either
                   synthetic or non-synthetic and are increasingly used by
                   journalists, web platforms, and the general public to
                   identify misinformation and other forms of problematic
                   content. As both well-resourced organizations and the
                   non-technical general public generate more sophisticated
                   synthetic media, the capacity for purveyors of problematic
                   content to adapt induces a \textbackslashnewterm\{detection
                   dilemma\}: as detection practices become more accessible,
                   they become more easily circumvented. This paper describes
                   how a multistakeholder cohort from academia, technology
                   platforms, media entities, and civil society organizations
                   active in synthetic media detection and its socio-technical
                   implications evaluates the detection dilemma. Specifically,
                   we offer an assessment of detection contexts and adversary
                   capacities sourced from the broader, global AI and media
                   integrity community concerned with mitigating the spread of
                   harmful synthetic media. A collection of personas
                   illustrates the intersection between unsophisticated and
                   highly-resourced sponsors of misinformation in the context
                   of their technical capacities. This work concludes that
                   there is no ``best'' approach to navigating the detector
                   dilemma, but derives a set of implications from
                   multistakeholder input to better inform detection process
                   decisions and policies, in practice.",
  month         =  feb,
  year          =  2021,
  url           = "http://arxiv.org/abs/2102.06109",
  archivePrefix = "arXiv",
  eprint        = "2102.06109",
  primaryClass  = "cs.CY",
  arxivid       = "2102.06109",
  doi           = "10.48550/arXiv.2102.06109"
}

@ARTICLE{Wei2022-fa,
  title         = "Emergent Abilities of Large Language Models",
  author        = "Wei, Jason and Tay, Yi and Bommasani, Rishi and Raffel,
                   Colin and Zoph, Barret and Borgeaud, Sebastian and Yogatama,
                   Dani and Bosma, Maarten and Zhou, Denny and Metzler, Donald
                   and Chi, Ed H and Hashimoto, Tatsunori and Vinyals, Oriol
                   and Liang, Percy and Dean, Jeff and Fedus, William",
  abstract      = "Scaling up language models has been shown to predictably
                   improve performance and sample efficiency on a wide range of
                   downstream tasks. This paper instead discusses an
                   unpredictable phenomenon that we refer to as emergent
                   abilities of large language models. We consider an ability
                   to be emergent if it is not present in smaller models but is
                   present in larger models. Thus, emergent abilities cannot be
                   predicted simply by extrapolating the performance of smaller
                   models. The existence of such emergence implies that
                   additional scaling could further expand the range of
                   capabilities of language models.",
  month         =  jun,
  year          =  2022,
  url           = "http://arxiv.org/abs/2206.07682",
  archivePrefix = "arXiv",
  eprint        = "2206.07682",
  primaryClass  = "cs.CL",
  arxivid       = "2206.07682",
  doi           = "10.48550/arXiv.2206.07682"
}

@ARTICLE{Ji2023-rr,
  title     = "Survey of Hallucination in Natural Language Generation",
  author    = "Ji, Ziwei and Lee, Nayeon and Frieske, Rita and Yu, Tiezheng and
               Su, Dan and Xu, Yan and Ishii, Etsuko and Bang, Ye Jin and
               Madotto, Andrea and Fung, Pascale",
  abstract  = "Natural Language Generation (NLG) has improved exponentially in
               recent years thanks to the development of sequence-to-sequence
               deep learning technologies such as Transformer-based language
               models. This advancement has led to more fluent and coherent
               NLG, leading to improved development in downstream tasks such as
               abstractive summarization, dialogue generation, and data-to-text
               generation. However, it is also apparent that deep learning
               based generation is prone to hallucinate unintended text, which
               degrades the system performance and fails to meet user
               expectations in many real-world scenarios. To address this
               issue, many studies have been presented in measuring and
               mitigating hallucinated texts, but these have never been
               reviewed in a comprehensive manner before.In this survey, we
               thus provide a broad overview of the research progress and
               challenges in the hallucination problem in NLG. The survey is
               organized into two parts: (1) a general overview of metrics,
               mitigation methods, and future directions, and (2) an overview
               of task-specific research progress on hallucinations in the
               following downstream tasks, namely abstractive summarization,
               dialogue generation, generative question answering, data-to-text
               generation, and machine translation. This survey serves to
               facilitate collaborative efforts among researchers in tackling
               the challenge of hallucinated texts in NLG.",
  journal   = "ACM Comput. Surv.",
  publisher = "Association for Computing Machinery",
  volume    =  55,
  number    =  12,
  pages     = "1--38",
  month     =  mar,
  year      =  2023,
  url       = "https://doi.org/10.1145/3571730",
  address   = "New York, NY, USA",
  keywords  = "Hallucination, intrinsic hallucination, extrinsic hallucination,
               faithfulness in NLG, factuality in NLG, consistency in NLG",
  issn      = "0360-0300",
  doi       = "10.1145/3571730"
}

@ARTICLE{Harris2023-na,
  title    = "Liars and Trolls and Bots Online: The Problem of Fake Persons",
  author   = "Harris, Keith Raymond",
  abstract = "This paper describes the ways in which trolls and bots impede the
              acquisition of knowledge online. I distinguish between three ways
              in which trolls and bots can impede knowledge acquisition,
              namely, by deceiving, by encouraging misplaced skepticism, and by
              interfering with the acquisition of warrant concerning persons
              and content encountered online. I argue that these threats are
              difficult to resist simultaneously. I argue, further, that the
              threat that trolls and bots pose to knowledge acquisition goes
              beyond the mere threat of online misinformation, or the more
              familiar threat posed by liars offline. Trolls and bots are, in
              effect, fake persons. Consequently, trolls and bots can
              systemically interfere with knowledge acquisition by manipulating
              the signals whereby individuals acquire knowledge from one
              another online. I conclude with a brief discussion of some
              possible remedies for the problem of fake persons.",
  journal  = "Philos. Technol.",
  volume   =  36,
  number   =  2,
  pages    = "35",
  month    =  may,
  year     =  2023,
  url      = "https://doi.org/10.1007/s13347-023-00640-9",
  issn     = "2210-5433",
  doi      = "10.1007/s13347-023-00640-9"
}

% The entry below contains non-ASCII chars that could not be converted
% to a LaTeX equivalent.
@ARTICLE{Gorwa2020-ye,
  title     = "Unpacking the social media bot: A typology to guide research and
               policy",
  author    = "Gorwa, Robert and Guilbeault, Douglas",
  abstract  = "Amid widespread reports of digital influence operations during
               major elections, policymakers, scholars, and journalists have
               become increasingly interested in the political impact of social
               media bots. Most recently, platform companies like Facebook and
               Twitter have been summoned to testify about bots as part of
               investigations into digitally enabled foreign manipulation
               during the 2016 U.S. Presidential election. Facing mounting
               pressure from both the public and from legislators, these
               companies have been instructed to crack down on apparently
               malicious bot accounts. But as this article demonstrates, since
               the earliest writings on bots in the 1990s, there has been
               substantial confusion as to exactly what a ``bot'' is and what
               it does. We argue that multiple forms of ambiguity are
               responsible for much of the complexity underlying contemporary
               bot‐related policy, and that before successful policy
               interventions can be formulated, a more comprehensive
               understanding of bots---especially how they are defined and
               measured---will be needed. In this article, we provide a
               typology of different types of bots, provide clear guidelines
               for better categorizing political automation, and unpack the
               impact that it can have on contemporary technology policy. We
               conclude by outlining the main challenges and ambiguities that
               will face both researchers and legislators as they tackle bots
               in the future.",
  journal   = "Policy Internet",
  publisher = "Wiley",
  volume    =  12,
  number    =  2,
  pages     = "225--248",
  month     =  jun,
  year      =  2020,
  url       = "http://doi.org/10.1002/poi3.184",
  copyright = "http://onlinelibrary.wiley.com/termsAndConditions\#vor",
  language  = "en",
  issn      = "2194-6019, 1944-2866",
  doi       = "10.1002/poi3.184"
}

@ARTICLE{Goldstein2023-kk,
  title         = "Generative Language Models and Automated Influence
                   Operations: Emerging Threats and Potential Mitigations",
  author        = "Goldstein, Josh A and Sastry, Girish and Musser, Micah and
                   DiResta, Renee and Gentzel, Matthew and Sedova, Katerina",
  abstract      = "Generative language models have improved drastically, and
                   can now produce realistic text outputs that are difficult to
                   distinguish from human-written content. For malicious
                   actors, these language models bring the promise of
                   automating the creation of convincing and misleading text
                   for use in influence operations. This report assesses how
                   language models might change influence operations in the
                   future, and what steps can be taken to mitigate this threat.
                   We lay out possible changes to the actors, behaviors, and
                   content of online influence operations, and provide a
                   framework for stages of the language model-to-influence
                   operations pipeline that mitigations could target (model
                   construction, model access, content dissemination, and
                   belief formation). While no reasonable mitigation can be
                   expected to fully prevent the threat of AI-enabled influence
                   operations, a combination of multiple mitigations may make
                   an important difference.",
  month         =  jan,
  year          =  2023,
  url           = "http://arxiv.org/abs/2301.04246",
  archivePrefix = "arXiv",
  eprint        = "2301.04246",
  primaryClass  = "cs.CY",
  arxivid       = "2301.04246",
  doi           = "10.48550/arXiv.2301.04246"
}

@ARTICLE{Golda2024-fy,
  title     = "Privacy and Security Concerns in Generative {AI}: A
               Comprehensive Survey",
  author    = "Golda, Abenezer and Mekonen, Kidus and Pandey, Amit and Singh,
               Anushka and Hassija, Vikas and Chamola, Vinay and Sikdar, Biplab",
  abstract  = "Generative Artificial Intelligence (GAI) has sparked a
               transformative wave across various domains, including machine
               learning, healthcare, business, and entertainment, owing to its
               remarkable ability to generate lifelike data. This comprehensive
               survey offers a meticulous examination of the privacy and
               security challenges inherent to GAI. It provides five pivotal
               perspectives essential for a comprehensive understanding of
               these intricacies. The paper encompasses discussions on GAI
               architectures, diverse generative model types, practical
               applications, and recent advancements within the field. In
               addition, it highlights current security strategies and proposes
               sustainable solutions, emphasizing user, developer,
               institutional, and policymaker involvement.",
  journal   = "IEEE Access",
  publisher = "IEEE",
  volume    =  12,
  pages     = "48126--48144",
  year      =  2024,
  url       = "http://doi.org/10.1109/ACCESS.2024.3381611",
  issn      = "2169-3536",
  doi       = "10.1109/ACCESS.2024.3381611"
}

@ARTICLE{Gartlehner2023-jw,
  title    = "Data extraction for evidence synthesis using a large language
              model: A proof-of-concept study",
  author   = "Gartlehner, G and Kahwati, L and Hilscher, R and Thomas, I and
              Kugley, S and Crotty, K and Viswanathan, M and Nussbaumer-Streit,
              B and Booth, G and Erskine, N and Konet, A and Chew, R",
  abstract = "Data extraction is a crucial, yet labor-intensive and error-prone
              part of evidence synthesis. To date, efforts to harness machine
              learning for enhancing efficiency of the data extraction process
              have fallen short of achieving sufficient accuracy and usability.
              With the advent of Large Language Models (LLMs), new
              possibilities have emerged to increase efficiency and accuracy of
              data extraction for evidence synthesis. The objective of this
              proof-of-concept study was to assess the performance of an LLM
              (Claude 2) in extracting data elements from published studies,
              compared with human data extraction as employed in systematic
              reviews. Our analysis utilized a convenience sample of 10
              English-language, open-access publications of randomized
              controlled trials included in a single systematic review. We
              selected 16 distinct types of data, posing varying degrees of
              difficulty (160 data elements across 10 studies). We used the
              browser version of Claude 2 to upload the portable document
              format of each publication and then prompted the model for each
              data element. Across 160 data elements, Claude 2 demonstrated an
              overall accuracy of 96.3\% with a high test-retest reliability
              (replication 1: 96.9\%; replication 2: 95.0\% accuracy). Overall,
              Claude 2 made 6 errors on 160 data items. The most common errors
              (n=4) were missed data items. Importantly, Claude 2's ease of use
              was high; it required no technical expertise or training data for
              effective operation. Based on findings of our proof-of-concept
              study, leveraging LLMs has the potential to substantially enhance
              the efficiency and accuracy of data extraction for evidence
              syntheses.",
  month    =  oct,
  year     =  2023,
  url      = "https://www.medrxiv.org/content/10.1101/2023.10.02.23296415v1",
  doi      = "10.1101/2023.10.02.23296415"
}

@ARTICLE{Feuerriegel2023-eg,
  title    = "Research can help to tackle {AI-generated} disinformation",
  author   = "Feuerriegel, Stefan and DiResta, Ren{\'e}e and Goldstein, Josh A
              and Kumar, Srijan and Lorenz-Spreen, Philipp and Tomz, Michael
              and Pr{\"o}llochs, Nicolas",
  journal  = "Nat Hum Behav",
  volume   =  7,
  number   =  11,
  pages    = "1818--1821",
  month    =  nov,
  year     =  2023,
  url      = "http://doi.org/10.1038/s41562-023-01726-2",
  language = "en",
  issn     = "2397-3374",
  pmid     = "37985906",
  doi      = "10.1038/s41562-023-01726-2"
}

@ARTICLE{Ferrara2024-bv,
  title    = "{GenAI} against humanity: nefarious applications of generative
              artificial intelligence and large language models",
  author   = "Ferrara, Emilio",
  abstract = "Generative Artificial Intelligence (GenAI) and Large Language
              Models (LLMs) are marvels of technology; celebrated for their
              prowess in natural language processing and multimodal content
              generation, they promise a transformative future. But as with all
              powerful tools, they come with their shadows. Picture living in a
              world where deepfakes are indistinguishable from reality, where
              synthetic identities orchestrate malicious campaigns, and where
              targeted misinformation or scams are crafted with unparalleled
              precision. Welcome to the darker side of GenAI applications. This
              article is not just a journey through the meanders of potential
              misuse of GenAI and LLMs, but also a call to recognize the
              urgency of the challenges ahead. As we navigate the seas of
              misinformation campaigns, malicious content generation, and the
              eerie creation of sophisticated malware, we'll uncover the
              societal implications that ripple through the GenAI revolution we
              are witnessing. From AI-powered botnets on social media platforms
              to the unnerving potential of AI to generate fabricated
              identities, or alibis made of synthetic realities, the stakes
              have never been higher. The lines between the virtual and the
              real worlds are blurring, and the consequences of potential
              GenAI's nefarious applications impact us all. This article serves
              both as a synthesis of rigorous research presented on the risks
              of GenAI and misuse of LLMs and as a thought-provoking vision of
              the different types of harmful GenAI applications we might
              encounter in the near future, and some ways we can prepare for
              them.",
  journal  = "Journal of Computational Social Science",
  month    =  feb,
  year     =  2024,
  url      = "https://doi.org/10.1007/s42001-024-00250-1",
  issn     = "2432-2725",
  doi      = "10.1007/s42001-024-00250-1"
}

@ARTICLE{Cooke2024-tb,
  title         = "As Good As A Coin Toss: Human detection of {AI-generated}
                   images, videos, audio, and audiovisual stimuli",
  author        = "Cooke, Di and Edwards, Abigail and Barkoff, Sophia and
                   Kelly, Kathryn",
  abstract      = "As synthetic media becomes progressively more realistic and
                   barriers to using it continue to lower, the technology has
                   been increasingly utilized for malicious purposes, from
                   financial fraud to nonconsensual pornography. Today, the
                   principal defense against being misled by synthetic media
                   relies on the ability of the human observer to visually and
                   auditorily discern between real and fake. However, it
                   remains unclear just how vulnerable people actually are to
                   deceptive synthetic media in the course of their day to day
                   lives. We conducted a perceptual study with 1276
                   participants to assess how accurate people were at
                   distinguishing synthetic images, audio only, video only, and
                   audiovisual stimuli from authentic. To reflect the
                   circumstances under which people would likely encounter
                   synthetic media in the wild, testing conditions and stimuli
                   emulated a typical online platform, while all synthetic
                   media used in the survey was sourced from publicly
                   accessible generative AI technology. We find that overall,
                   participants struggled to meaningfully discern between
                   synthetic and authentic content. We also find that detection
                   performance worsens when the stimuli contains synthetic
                   content as compared to authentic content, images featuring
                   human faces as compared to non face objects, a single
                   modality as compared to multimodal stimuli, mixed
                   authenticity as compared to being fully synthetic for
                   audiovisual stimuli, and features foreign languages as
                   compared to languages the observer is fluent in. Finally, we
                   also find that prior knowledge of synthetic media does not
                   meaningfully impact their detection performance.
                   Collectively, these results indicate that people are highly
                   susceptible to being tricked by synthetic media in their
                   daily lives and that human perceptual detection capabilities
                   can no longer be relied upon as an effective counterdefense.",
  month         =  mar,
  year          =  2024,
  url           = "http://arxiv.org/abs/2403.16760",
  archivePrefix = "arXiv",
  eprint        = "2403.16760",
  primaryClass  = "cs.HC",
  arxivid       = "2403.16760",
  doi           = "10.48550/arXiv.2403.16760"
}

@ARTICLE{Chao2023-dn,
  title         = "Jailbreaking Black Box Large Language Models in Twenty
                   Queries",
  author        = "Chao, Patrick and Robey, Alexander and Dobriban, Edgar and
                   Hassani, Hamed and Pappas, George J and Wong, Eric",
  abstract      = "There is growing interest in ensuring that large language
                   models (LLMs) align with human values. However, the
                   alignment of such models is vulnerable to adversarial
                   jailbreaks, which coax LLMs into overriding their safety
                   guardrails. The identification of these vulnerabilities is
                   therefore instrumental in understanding inherent weaknesses
                   and preventing future misuse. To this end, we propose Prompt
                   Automatic Iterative Refinement (PAIR), an algorithm that
                   generates semantic jailbreaks with only black-box access to
                   an LLM. PAIR -- which is inspired by social engineering
                   attacks -- uses an attacker LLM to automatically generate
                   jailbreaks for a separate targeted LLM without human
                   intervention. In this way, the attacker LLM iteratively
                   queries the target LLM to update and refine a candidate
                   jailbreak. Empirically, PAIR often requires fewer than
                   twenty queries to produce a jailbreak, which is orders of
                   magnitude more efficient than existing algorithms. PAIR also
                   achieves competitive jailbreaking success rates and
                   transferability on open and closed-source LLMs, including
                   GPT-3.5/4, Vicuna, and PaLM-2.",
  month         =  oct,
  year          =  2023,
  url           = "http://arxiv.org/abs/2310.08419",
  archivePrefix = "arXiv",
  eprint        = "2310.08419",
  primaryClass  = "cs.LG",
  arxivid       = "2310.08419",
  doi           = "10.48550/arXiv.2310.08419"
}

@ARTICLE{Carlini2023-yv,
  title         = "Poisoning {Web-Scale} Training Datasets is Practical",
  author        = "Carlini, Nicholas and Jagielski, Matthew and Choquette-Choo,
                   Christopher A and Paleka, Daniel and Pearce, Will and
                   Anderson, Hyrum and Terzis, Andreas and Thomas, Kurt and
                   Tram{\`e}r, Florian",
  abstract      = "Deep learning models are often trained on distributed,
                   web-scale datasets crawled from the internet. In this paper,
                   we introduce two new dataset poisoning attacks that
                   intentionally introduce malicious examples to a model's
                   performance. Our attacks are immediately practical and
                   could, today, poison 10 popular datasets. Our first attack,
                   split-view poisoning, exploits the mutable nature of
                   internet content to ensure a dataset annotator's initial
                   view of the dataset differs from the view downloaded by
                   subsequent clients. By exploiting specific invalid trust
                   assumptions, we show how we could have poisoned 0.01\% of
                   the LAION-400M or COYO-700M datasets for just \$60 USD. Our
                   second attack, frontrunning poisoning, targets web-scale
                   datasets that periodically snapshot crowd-sourced content --
                   such as Wikipedia -- where an attacker only needs a
                   time-limited window to inject malicious examples. In light
                   of both attacks, we notify the maintainers of each affected
                   dataset and recommended several low-overhead defenses.",
  month         =  feb,
  year          =  2023,
  url           = "http://arxiv.org/abs/2302.10149",
  archivePrefix = "arXiv",
  eprint        = "2302.10149",
  primaryClass  = "cs.CR",
  arxivid       = "2302.10149",
  doi           = "10.48550/arXiv.2302.10149"
}

@ARTICLE{Brundage2018-pk,
  title         = "The Malicious Use of Artificial Intelligence: Forecasting,
                   Prevention, and Mitigation",
  author        = "Brundage, Miles and Avin, Shahar and Clark, Jack and Toner,
                   Helen and Eckersley, Peter and Garfinkel, Ben and Dafoe,
                   Allan and Scharre, Paul and Zeitzoff, Thomas and Filar,
                   Bobby and Anderson, Hyrum and Roff, Heather and Allen,
                   Gregory C and Steinhardt, Jacob and Flynn, Carrick and
                   h{\'E}igeartaigh, Se{\'a}n {\'O} and Beard, Simon and
                   Belfield, Haydn and Farquhar, Sebastian and Lyle, Clare and
                   Crootof, Rebecca and Evans, Owain and Page, Michael and
                   Bryson, Joanna and Yampolskiy, Roman and Amodei, Dario",
  abstract      = "This report surveys the landscape of potential security
                   threats from malicious uses of AI, and proposes ways to
                   better forecast, prevent, and mitigate these threats. After
                   analyzing the ways in which AI may influence the threat
                   landscape in the digital, physical, and political domains,
                   we make four high-level recommendations for AI researchers
                   and other stakeholders. We also suggest several promising
                   areas for further research that could expand the portfolio
                   of defenses, or make attacks less effective or harder to
                   execute. Finally, we discuss, but do not conclusively
                   resolve, the long-term equilibrium of attackers and
                   defenders.",
  month         =  feb,
  year          =  2018,
  url           = "http://arxiv.org/abs/1802.07228",
  archivePrefix = "arXiv",
  eprint        = "1802.07228",
  primaryClass  = "cs.AI",
  arxivid       = "1802.07228",
  doi           = "10.48550/arXiv.1802.07228"
}

@ARTICLE{Bright2024-zs,
  title         = "Generative {AI} is already widespread in the public sector",
  author        = "Bright, Jonathan and Enock, Florence E and Esnaashari, Saba
                   and Francis, John and Hashem, Youmna and Morgan, Deborah",
  abstract      = "Generative AI has the potential to transform how public
                   services are delivered by enhancing productivity and
                   reducing time spent on bureaucracy. Furthermore, unlike
                   other types of artificial intelligence, it is a technology
                   that has quickly become widely available for bottom-up
                   adoption: essentially anyone can decide to make use of it in
                   their day to day work. But to what extent is generative AI
                   already in use in the public sector? Our survey of 938
                   public service professionals within the UK (covering
                   education, health, social work and emergency services) seeks
                   to answer this question. We find that use of generative AI
                   systems is already widespread: 45\% of respondents were
                   aware of generative AI usage within their area of work,
                   while 22\% actively use a generative AI system. Public
                   sector professionals were positive about both current use of
                   the technology and its potential to enhance their efficiency
                   and reduce bureaucratic workload in the future. For example,
                   those working in the NHS thought that time spent on
                   bureaucracy could drop from 50\% to 30\% if generative AI
                   was properly exploited, an equivalent of one day per week
                   (an enormous potential impact). Our survey also found a high
                   amount of trust (61\%) around generative AI outputs, and a
                   low fear of replacement (16\%). While respondents were
                   optimistic overall, areas of concern included feeling like
                   the UK is missing out on opportunities to use AI to improve
                   public services (76\%), and only a minority of respondents
                   (32\%) felt like there was clear guidance on generative AI
                   usage in their workplaces. In other words, it is clear that
                   generative AI is already transforming the public sector, but
                   uptake is happening in a disorganised fashion without clear
                   guidelines. The UK's public sector urgently needs to develop
                   more systematic methods for taking advantage of the
                   technology.",
  month         =  jan,
  year          =  2024,
  url           = "http://arxiv.org/abs/2401.01291",
  archivePrefix = "arXiv",
  eprint        = "2401.01291",
  primaryClass  = "cs.CY",
  arxivid       = "2401.01291",
  doi           = "10.48550/arXiv.2401.01291"
}

@ARTICLE{Blauth2022-vl,
  title     = "Artificial Intelligence Crime: An Overview of Malicious Use and
               Abuse of {AI}",
  author    = "Blauth, Ta{\'\i}s Fernanda and Gstrein, Oskar Josef and Zwitter,
               Andrej",
  abstract  = "The capabilities of Artificial Intelligence (AI) evolve rapidly
               and affect almost all sectors of society. AI has been
               increasingly integrated into criminal and harmful activities,
               expanding existing vulnerabilities, and introducing new threats.
               This article reviews the relevant literature, reports, and
               representative incidents which allows to construct a typology of
               the malicious use and abuse of systems with AI capabilities. The
               main objective is to clarify the types of activities and
               corresponding risks. Our starting point is to identify the
               vulnerabilities of AI models and outline how malicious actors
               can abuse them. Subsequently, we explore AI-enabled and
               AI-enhanced attacks. While we present a comprehensive overview,
               we do not aim for a conclusive and exhaustive classification.
               Rather, we provide an overview of the risks of enhanced AI
               application, that contributes to the growing body of knowledge
               on the issue. Specifically, we suggest four types of malicious
               abuse of AI (integrity attacks, unintended AI outcomes,
               algorithmic trading, membership inference attacks) and four
               types of malicious use of AI (social engineering,
               misinformation/fake news, hacking, autonomous weapon systems).
               Mapping these threats enables advanced reflection of governance
               strategies, policies, and activities that can be developed or
               improved to minimize risks and avoid harmful consequences.
               Enhanced collaboration among governments, industries, and civil
               society actors is vital to increase preparedness and resilience
               against malicious use and abuse of AI.",
  journal   = "IEEE Access",
  publisher = "IEEE",
  volume    =  10,
  pages     = "77110--77122",
  year      =  2022,
  url       = "http://doi.org/10.1109/ACCESS.2022.3191790",
  issn      = "2169-3536",
  doi       = "10.1109/ACCESS.2022.3191790"
}

@ARTICLE{Barrett2023-gv,
  title     = "Identifying and Mitigating the Security Risks of Generative {AI}",
  author    = "Barrett, Clark and Boyd, Brad and Bursztein, Elie and Carlini,
               Nicholas and Chen, Brad and Choi, Jihye and Chowdhury, Amrita
               Roy and Christodorescu, Mihai and Datta, Anupam and Feizi,
               Soheil and Fisher, Kathleen and Hashimoto, Tatsunori and
               Hendrycks, Dan and Jha, Somesh and Kang, Daniel and Kerschbaum,
               Florian and Mitchell, Eric and Mitchell, John and Ramzan,
               Zulfikar and Shams, Khawaja and Song, Dawn and Taly, Ankur and
               Yang, Diyi",
  journal   = "Foundations and Trends\textregistered{} in Privacy and Security",
  publisher = "Now Publishers",
  volume    =  6,
  number    =  1,
  pages     = "1--52",
  year      =  2023,
  url       = "http://doi.org/10.1561/3300000041",
  keywords  = "Security and privacy policies; Security architectures; Human
               factors in security and privacy; Artificial intelligence methods
               in security and privacy; Robustness; Behavioral, cognitive and
               neural learning; Deep learning",
  issn      = "2474-1558",
  doi       = "10.1561/3300000041"
}

@ARTICLE{Anderljung2023-ba,
  title         = "Protecting Society from {AI} Misuse: When are Restrictions
                   on Capabilities Warranted?",
  author        = "Anderljung, Markus and Hazell, Julian",
  abstract      = "Artificial intelligence (AI) systems will increasingly be
                   used to cause harm as they grow more capable. In fact, AI
                   systems are already starting to be used to automate
                   fraudulent activities, violate human rights, create harmful
                   fake images, and identify dangerous toxins. To prevent some
                   misuses of AI, we argue that targeted interventions on
                   certain capabilities will be warranted. These restrictions
                   may include controlling who can access certain types of AI
                   models, what they can be used for, whether outputs are
                   filtered or can be traced back to their user, and the
                   resources needed to develop them. We also contend that some
                   restrictions on non-AI capabilities needed to cause harm
                   will be required. Though capability restrictions risk
                   reducing use more than misuse (facing an unfavorable
                   Misuse-Use Tradeoff), we argue that interventions on
                   capabilities are warranted when other interventions are
                   insufficient, the potential harm from misuse is high, and
                   there are targeted ways to intervene on capabilities. We
                   provide a taxonomy of interventions that can reduce AI
                   misuse, focusing on the specific steps required for a misuse
                   to cause harm (the Misuse Chain), and a framework to
                   determine if an intervention is warranted. We apply this
                   reasoning to three examples: predicting novel toxins,
                   creating harmful images, and automating spear phishing
                   campaigns.",
  month         =  mar,
  year          =  2023,
  url           = "http://arxiv.org/abs/2303.09377",
  archivePrefix = "arXiv",
  eprint        = "2303.09377",
  primaryClass  = "cs.AI",
  arxivid       = "2303.09377",
  doi           = "10.48550/arXiv.2303.09377"
}

